A Survey of Safety and Trustworthiness of Deep Neural Networks: Verification, Testing, Adversarial Attack and Defence, and Interpretability

In the past few years, significant progress has been made on deep neural networks (DNNs) in achieving human-level performance on several long-standing tasks. With the broader deployment of DNNs on various applications, the concerns over their safety and trustworthiness have been raised in public, especially after the widely reported fatal incidents involving self-driving cars. Research to address these concerns is particularly active, with a significant number of papers released in the past few years. This survey paper conducts a review of the current research effort into making DNNs safe and trustworthy, by focusing on four aspects: verification, testing, adversarial attack and defence, and interpretability. In total, we survey 202 papers, most of which were published after 2017.

==> Interpretability.tex <==
\newpage
\section{Interpretability}
\label{sec:interpretability}

The interpretability (or explainability) has been an active area of research, due to the black-box nature of DNNs. DNNs have shown the ability of achieving high precision on their predictions. However, to gain the trust from human users, it is essential to enable human users to understand the decisions a DNN has made.   

\subsection{Visualisation}

The research on visualising DNNs aims to understand the representation learned by DNNs through visualisation. It  focuses on convolutional neural networks (CNNs) with images as their inputs, and is mainly for instance-wise explanation. 

\cite{EBCV2009} synthesises images that cause high activations for particular neurons by treating the synthesis problem as an optimisation problem.
\begin{equation}
x^* =\arg \max_{x} u_{k,l}(x)
\end{equation}
Recall that $ u_{k,l}(x)$ is the activation of the $l$-th neuron on the $k$-th layer for the input $x$. In general, the optimisation problem  is non-convex, and therefore a gradient ascent based algorithm is applied to find a local optimum. 
Starting with some initial input $x=x_0$, the activation $u_{k,l}(x)$  is computed, and then steps are taken in input space along the gradient ${\partial u_{k,l}(x)/{\partial x}}$ to synthesize inputs that cause higher and higher activations of for the neuron $n_{k,l}$, and eventually terminates at some $x^*$ which is deemed to be a preferred input stimulus for the neuron in question. 


\cite{MV2014} computes an approximate inverse of an image representation. Let  $\explain:\real^{s_1} \rightarrow \realnumber^{a_1}$ be a representation function, mapping an input to a  representation of $a_1$ dimensions. Now given a representation $T_0$ to be inverted, it is to find an input $x^*$ such that 
\begin{equation}\label{equ:invert}
x^* = \arg\min_{x\in \real^{s_1}} \lossfunction(\explain(x),T_0) + \lambda \regulariser(x)
\end{equation}
where $\lossfunction$ is a loss function comparing two representations, $\regulariser(x)$ is a regulariser, and $\lambda$ is a multiplier to balance between the two terms. For the loss function $\lossfunction$, Euclidean distance norm is taken. For the regulariser, they use either an image prior
\begin{equation}
\regulariser_\alpha(x) = \distance{x}{\alpha}^\alpha
\end{equation}
where $\alpha = 6$ is taken in their experiments, or a total variation, which encourages  images to consist of piece-wise constant
patches. 
For the algorithm to solve the above optimsation expression (\ref{equ:invert}), the gradient descent  procedure is extended to use momentum. 

\cite{DB2015} proposes to analyse which information is preserved by a feature representation and which information is discarded. Given a feature vector, it trains a DNN to predict the expected pre-image, i.e., the weighted average of all natural images which could have produced the given feature vector. Given a training set of images and their features $\{x_i,\phi_i\}$, it is to learn the weight $w$ of a network $f(\phi,w)$ to minimise a Monte-Carlo estimate of the loss as follows: 
\begin{equation}
\hat{w} = \arg\min_w \sum_i ||x_i - f(\phi_i,w) ||_2^2
\end{equation}


It has been argued \cite{YCNFL2015} that gradient-based approaches do not produce images that resemble natural images.



\subsection{Ranking}

The next major approaches are to compute a ranking of a set of features. Specifically, given an input $\inputPoint$ and a set $\features$ of features, it is to find a mapping $r_{\inputPoint}:\features\rightarrow \real$ 
%
such that each feature $\feature\in \features$ has a rank $r_\inputPoint(\feature)$. Intuitively, the ranking $r_\inputPoint$ provides a total order between features on their contributions to a decision making of $\network$ on the input $\inputPoint$. 



\subsubsection{LIME}

LIME \cite{LIME} interprets individual model prediction by locally approximating the model around a given prediction. Given an image $x$, LIME treats it as a set of superpixels, and to compute the rank, it minimises over the following objective function: 
%
\begin{equation}
{\cal E} = \arg\min_{g\in {\cal G}} \lossfunction(f,g,\pi_{x'}) + \regulariser(g)
\end{equation}
where $\lossfunction(f,g,\pi_{x'})$ is a loss of taking the explanation $g$ with respect to the original model $f$, under the condition of a local kernel $\pi_{x'}$. The reguralisation term $\regulariser(g)$ is to penalise the complexity of the explanation $g$. 
%The computation of the optimal value is done by taking algorithm to find 


\subsubsection{DeepLIFT}

\cite{SGK2017} is a recursive prediction explanation method. It attributes to each input $x_i$ a value $C_{\Delta x_i\Delta y}$ that represents the effect of that input being set to a reference value as opposed to its original value. The reference value, chosen by the user, represents a typical uninformative background value for the feature. DeepLIFT uses a ``summation-to-delta'' property that states: 
\begin{equation}
\sum_{i=1}^n C_{\Delta x_i\Delta y} = \Delta o, 
\end{equation}
where $o=f(x)$ is the method output, $\Delta o=f(x)-f(r)$, $\Delta x_i = x_i-r_i$, and $r$ is the reference input. 

\subsubsection{integrated gradient }

\cite{STY2017} suggests that a good explanation should satisfy the following two axiomatic attributes: 
\begin{itemize}
\item Sensitivity, which requires that for every input and baseline that differ in one feature but have different predictions then the differing feature should be given a non-zero attribution. 
\item Implementation invariance, which requires that the attributions are always identical for two functionally equivalent networks.
\end{itemize}

Based on these axiomatic attributes, they propose the integrated gradient and show that it is the canonical among path methods which are the only methods to satisfy certain desirable axioms including Sensitivity and Implementation invariance. Technically, the integrated gradient along the $i$-th dimension for an input $x$ and a baseline $x'$ is as follows.
\begin{equation}
IntegratedGrad_i(x) = (x_i-x_i')\times \int_{\alpha=0}^1 \frac{{\partial F(x'+\alpha\times(x-x'))}}{{\partial x_i}} d\alpha
\end{equation}
where $\frac{{\partial} F(x)}{{\partial x_i}}$ is the gradient of $F(x)$ along the $i$-th dimension. 

\subsubsection{layer-wise}

\cite{LMC2017} is equivalent to DeepLIFT with the reference activations of all neurons fixed to zero. 

\subsubsection{SHARPLEY}

\cite{LL2017} suggests take an additive model $$
g(z') = \phi_0 + \sum_{i=1}^M \phi_i z_i'
$$ 
as an explanation model, where $M$ is the number of simplified input features, $z'\in \{0,1\}^M$, and $\phi_i\in \mathbb{R}$ is a coefficient. It shows that under three properties (local accuracy, missingness, consistency), there is only one possible explanation model. 
\begin{equation}
\phi_i(f,x) = \sum_{z' \subseteq x'} \frac{|z'|! (M-|z'|-1)!}{M!} [f_x(z')-f_x(z'\setminus i)]
\end{equation}
where $|z'|$ is the number of non-zero entries in $z'$, and $z'\subseteq x'$ represents all $z'$ vectors where the non-zero entries are a subset of the non-zero entries in $x'$. 

\subsubsection{Concept Activation Vectors}

\cite{KWGCWVS2018} argues that, since most machine learning models operate on features, such as pixel values, that do not correspond to high-level concepts that humans understand, existing ranking-based approaches do not produce an explanation that can be easily accessible to humans. It then works on the idea of supplementing high level concepts (i.e., concept activation vector) into this explanation to make the  final explanation closer to human understandable explanation. The high-level concepts are learned independently from other user-provided data. 

%\subsubsection{Optimisation}

%\subsubsection{Highlight}


\subsection{Saliency Map (non-ranking based)}

\cite{ZF2013} highlights the portions of a particular image that are responsible for the firing of each neural unit. 


\subsection{Information Theory}

\cite{CSWJ2018} utilises an instancewise feature selection for model interpretation. Roughly speaking, for a given input $\inputPoint$, among a set of $n$ features, it is to choose $k$ most informative features. Let $\mathscr{P}_k=\{S\subset 2^n~|~|S| = k\}$ be the set of all subsets of size $k$. An explainer $\mathcal{E}$ of size $k$ is a mapping from the feature space $\real^n$ to the power set $\mathscr{P}_k$.  Then, the problem is to find a solution for the following optimsiation problem: 
\begin{equation}
\max_{\mathcal{E}} I(X_S;Y) \text{   subject to } S\sim \mathcal{E}(X)
\end{equation}
where $I(X_S;Y)$ represents the mutual information between features $X_S$ and the output $Y$. Intuitively, the explainer is to find a set of features to maximise the mutual information between selected features and the output. Because the problem is computationally hard to solve, a variational approximation is developed to compute it efficiently. 

\subsection{Influence Function}

\cite{KL2017} considers influence functions, a classic technique from robust statistics, to trace a model’s prediction through the
learning algorithm and back to its training data. Basically, it is done by e.g., upweighting a training point or perturbing a training point. 

\subsection{Linear Programming}

\cite{CHHWP2018} works with piecewise linear neural networks (PLNN), whose activation functions are piecewise linear such as ReLU. Given an input $x$, its corresponding activation pattern, i.e., the states of all hidden neurons, is fixed and equivalent to a set of linear inequalities. Each inequality represents a decision feature, and therefore the interpretation of $x$ includes all the decision features. Moreover, because all inputs sharing the same activation pattern form a unique convex polytope, the interpretation of an input $x$ can also include the the decision features of the polytope boundaries. 



==> images/concolic-flow.tex <==
\tikzstyle{decision} = [diamond, draw, fill=blue!20, 
    text width=4.5em, text badly centered, node distance=3cm, inner sep=0pt]
\tikzstyle{block} = [rectangle, draw, fill=blue!20, 
    text width=5em, text centered, rounded corners, minimum height=4em]
\tikzstyle{every node}=[font=\Large]
\tikzstyle{line} = [draw, -latex']
\tikzstyle{cloud} = [draw, ellipse,fill=red!20, node distance=3cm,
    minimum height=2em]

\begin{tikzpicture}[node distance = 2cm, auto]

  \node [] (init) {}; %$\{t_0\}$: the seed input};
  \node [above of=init, node distance=0.5cm, xshift=-0.2cm] (init2) {$\{t_0\}$: seed input};

  \node [decision, right of=init, node distance=2cm] (testsuite) {$\mathcal{T}$};
  
  \node [above of=init, node distance=5cm] (requirements) {};
  
  \node [above of=requirements, node distance=0.75cm, xshift=0.5cm, yshift=0.2cm] (requirements2) {
                                      \begin{tabular}{l}
                                        $\mathfrak{R}$: coverage requirements,\\$\delta$: a heuristic
                                      \end{tabular}
                                      };
  \node [block, right of=requirements, node distance=2cm] (requirements2) {$\delta(\mathfrak{R})$};
  
  \node [block, right of=testsuite, node distance=3cm, yshift=2.5cm] (concrete) {concrete execution};
  
  %\node [block, right of=concrete, node distance=4.5cm] (top-pair) {$(t,\delta(r))$};
  
  \node [block, right of=concrete, node distance=4.5cm] (top-pair) {$t, r$};
  
  \node [block, right of=top-pair, node distance=4.5cm] (testcase) {new input $t'$};

  \node [cloud, below of=testsuite, node distance=2.5cm] (oracle) {Oracle};
  
  \node [right of=oracle, node distance=4.5cm] (adversarials) {adversarial examples};
  
  \node [above of=top-pair, node distance=4cm, xshift=2.5cm] (algorithm) {\textbf{Algorithm 1}};

  


  % Draw edges
  \path [line, line width=0.3mm] (init) -- (testsuite);
  \path [line, line width=0.3mm] (requirements) -- (requirements2);
  \path [line, line width=0.3mm] (requirements2) -- (concrete);
  \path [line, line width=0.3mm] (testsuite) -- (concrete);
  \path [line, line width=0.3mm] (concrete) -- node[above]{top} node[below]{ranked} (top-pair);
  \path [line, line width=0.3mm] (top-pair) -- node[above]{symbolic} node[below]{analysis} (testcase);
  \path [line, line width=0.3mm] (testcase) |- (testsuite);
  \path [line, line width=0.3mm] (testsuite) -- (oracle);
  \path [line, line width=0.3mm] (oracle) --  (adversarials);
  
  \draw[loosely dashed] (-2.3,-1) rectangle (15.2,7);
  
\end{tikzpicture}

